Resummed Distribution Functions: Making Perturbation Theory Positive and Normalized

Fixed-order perturbative calculations for differential cross sections can suffer from non-physical artifacts: they can be non-positive, non-normalizable, and non-finite, none of which occur in experimental measurements. We propose a framework, the Resummed Distribution Function (RDF), that, given a perturbative calculation for an observable to some finite order in $\alpha_s$, will ``resum'' the expression in a way that is guaranteed to match the original expression order-by-order and be positive, normalized, and finite. Moreover, our ansatz parameterizes all possible finite, positive, and normalized completions consistent with the original fixed-order expression, which can include N$^n$LL resummed expressions. The RDF also enables a more direct notion of perturbative uncertainties, as we can directly vary higher-order parameters and treat them as nuisance parameters. We demonstrate the power of the RDF ansatz by matching to thrust to $\mathcal{O}(\alpha_s^3)$ and extracting $\alpha_s$ with perturbative uncertainties by fitting the RDF to ALEPH data.

==> old.tex <==

% \section{Matching}


% \Rikab{@Radha should I delete this section? I think we are outdated}

% Given a fixed order calculation $p_{\rm FO}(x|\alpha)$ of an observable $x$, or equivalently $p_{\rm FO}(t|\alpha)$ which differs by only a known Jacobian $t(x)$, we would like to constrain the coefficients $c_{mn}$ in our Ansatz:
% %
% \begin{align}
%     q(t|\alpha) = f'(t|\alpha) e^{-f(t|\alpha)}, 
% \end{align}
% %
% where
% %
% \begin{align}
%     f(t|\alpha) = \sum_{m \leq M, n \leq N} c_{mn} \alpha^m t^n. 
% \end{align}


% Note that $p_{\rm FO}$ is \emph{not} necessarily a polynomial in $t$ and $\alpha$. 
% %
% This is especially the case if there are non-singular terms in $x$, or due to effects in the running of $\alpha$.
% %
% However, we can still always write:
% %
% \begin{align}
%     p_{FO}(t, \alpha) =  \sum_{m\leq M,n \leq N} p_{mn} \alpha^m t^n + \mathcal{O}(\alpha^{M+1}, t^{N+1}),\label{eq:taylor_expand_FO}
% \end{align}
% %
% even if the order of the fixed-order calculation is less than $M$.
% %
% If no running is included, and only singular terms are considered, then \Eq{taylor_expand_FO} is exact. 
% %
% Otherwise, it is an approximation.

% Then, it is simple to extract the coefficients $c_{mn}$:
% %
% \begin{align}
%     c_{mn} = -\left[\log(1 - \sum_{m',n'}\frac{p_{m',n'-1}\alpha^{m'}t^{n'-1}}{n})\right]_{mn},
% \end{align}
% %
% where the subscript $[\,]_{mn}$ refers to the $mn$ component of the Taylor expansion, which is easy to extract algorithmically. 
% %
% The factors of $n-1$ and $\frac{1}{n}$ come from integrating \Eq{taylor_expand_FO}.


% The resulting $c$'s are \emph{not} guaranteed to be a valid probability distribution, but it can happen.


% \subsection{Enforcing positivity}

% We would like the function $f'(t, \alpha)$ to be nonnegative whenever $t \geq 0$ and $\alpha \geq 0$. 
% %
% Moreover, for matching, we would like $f'$ to be analytic near $\alpha = 0$, with (preferably) as large a radius of convergence as possible.
% %
% That is, $f'$ should have a Taylor series:
% %
% \begin{align}
%     f' &= \sum_{m = 0} f'_m(t) \alpha^m \\
%     &= \sum_{m=0}^M f'_m(t) \alpha^m + \alpha^{M+1}h(t, \alpha)
% \end{align}
% %
% for some analytic $h$. Immediately, we know that the coefficients $f'_m$ must be real, but they need not be positive. 
% %
% Without loss of generality, we know that $f'_0$ can be set to 1 by dividing out factors.

% \subsection{Matching terms allowed}

% \textbf{Fixed coefficients.} \Radha{Added 02/04} Let's say I have a FO pdf with coefficients $p_{mn}$. Each power $\alpha^m$ will have a maximum $t$ power, which we can write as $t_{m_\mathrm{max}}$. For that power  $\alpha^m$, the maximum coefficient I can fix is $c_{m, t_{m_\mathrm{max}} + 1}$. 

% Now let's say I have a FO pdf with coefficients $p_{10}$, $p_{11}$, $p_{21}$, i.e. the pdf is $p_{10}\alpha + p_{11} \alpha t + p_{21}\alpha^2t$. I am allowed to fix $c_{10}$, $c_{11}$, $c_{12}$ and $c_{20}$, $c_{21}$.
% \\
% \\
% \Radha{The issue I was trying to outline}. Let's say that the FO pdf didn't have $p_{21}$ because the theory calculation wasn't done, \textit{not} because that term should be zero. If we assume that the ``theory truth" has a nonzero $p_{21}$, then we need to somehow learn a nonzero $c_{22}$. This can't be done during determination of the fixed coefficients, since we can only fix up to $c_{21}$. 

% If we enforce derivative matching up to order $\alpha^2$ to determine the non-fixed coefficients, then will this assign a non-zero value for $c_{22}$? If it doesn't, when do we turn on $c_{22}$?






% \section{Full example: Thrust}

% Thrust\Rikab{CITE} is an event-level IRC-safe observable.
% %
% It is defined as:
% %
% \begin{align}
%     T = 
% \end{align}
% %
% It is common to work with $\tau = 1 - T$ instead, so that its dynamic range is $[0, \frac{1}{2}]$.
% %
% The thrust distribution as measured by OPAL\Rikab{cite}, plus the fixed order calculations, are shown in \Fig{thrust_distribution}.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{Figures/thrust_opal.pdf}
%     \caption{Thrust Distribution}
% \label{fig:thrust_distribution}
% \end{figure}

% To first order in $\alpha_s$, ignoring terms that go to 0 as $\tau \to 0$, we have:
% %
% \begin{align}
%     \dv{\sigma}{\tau} = \frac{\alpha}{2\pi}C_F \frac{1}{\tau}(4\log\frac{1}{\tau} - 3).
% \end{align}
% %
% Note that the fixed order calculation goes negative at $\tau = e^{-3/4} \approx 0.472$.
% %
% This is because to first order in perturbation theory, it is not possible to generate configurations that saturate the $\tau = \frac{1}{2}$ bound. 
% %
% We cannot naively choose $t = \log\frac{1}{\tau}$ here, or even $t = \log\frac{1}{2\tau}$. 
% %
% This is because at $t = 0$, which is where our Taylor expansion begins, we will have $\dv{\sigma}{t}  <0$. 
% %
% No amount of additional terms can fix this, because the Taylor expansion is exact at $t = 0$.
% %
% We will need to choose a smarter $t$.

% \textbf{Method 1}: Following \Reference{Catani:1992ua}, we choose:
% %
% \begin{align}
%     t &= \log(\frac{1}{\tau} - \frac{1}{\tau_{\max}} + 1)\nonumber \\
%     &\updownarrow \nonumber \\
%     \tau &= \frac{\tau_{\max}}{\tau_{\max}(e^t-1) + 1}
% \end{align}
% %
% The Jacobian is:
% %
% \begin{align}
%     \left|\dv{\tau}{t}\right| &= \frac{\tau_{\max} e^t}{(\tau_{\max}(e^t-1) + 1)^2} \nonumber\\
%     &= \tau \frac{e^t}{\tau_{\max}(e^t-1) + 1}
% \end{align}


% %
% Then, we have:
% %
% \begin{align}
%     \dv{\sigma}{t} &= \frac{\alpha_s}{2\pi}C_F \left(\frac{e^t}{\tau_{\max}(e^t-1) + 1}\right)\left(4\log(1 + \tau_{\max}(e^t -1)) - 4\log(\tau_\max) - 3\right)\\
%     &= \frac{\alpha_s}{2\pi}C_F \left(\frac{e^t}{\tau_{\max}(e^t-1) + 1}\right)\left(4\log(1 - e^{-\frac{3}{4}} + e^{t-\frac{3}{4}} ))\right)
% \end{align}
% %
% When $t = 0$, we now have the PDF = 0. 
% %
% While this expression is extremely complicated, it goes to $0$ as $t\to 0$ and $\alpha \to 0$.
% %
% Therefore, we know the final answer can be written as:
% %
% \begin{align}
%     q(t|\alpha) = \alpha t e^{-g \dots}
% \end{align}
% %
% where the term in front of the exponentials are the $g^*$ terms.
% %
% We can rest easy knowing that whatever complicated stuff happens in the exponential, near 0, the $\alpha t$ dominates the behavior.




% To second order in $\alpha_s$, ignoring terms that go to 0 as $\tau \to 0$, we have:
% %
% \begin{align}
%     \dv{\sigma}{\tau} &= \left(\frac{\alpha C_F}{2\pi}\right) \frac{1}{\tau}(4\log\frac{1}{\tau} - 3) \nonumber\\
%     &+ \left(\frac{\alpha C_F}{2\pi}\right)^2\frac{1}{\tau}\left(8\log^3(\frac{1}{\tau}) + 18\log^2 + (13-4\pi^2)\log + \frac{9}{4} - 2\pi^2 + 4\zeta_3\right)
% \end{align}
% %
% Now, $\tau_{\max}$ is a function of $\alpha$. As $\alpha \to 0$, $\tau_{\max} \to e^{-3/4}$, but for larger values of $\alpha$, the max increases.
% %
% Therefore, no matter how we choose the shift, there will \emph{always} be a term that goes like $\alpha^m t^0$. 
% %
% If we choose the same shift as before (to kill all constants in $\alpha^1$), we will find that the lowest-order coefficient in the whole expression is $p_{20}\alpha^2 t^0$.
% %
% There is nothing inherently wrong with this.
% %
% But it is unpleasant that we cannot extract out the lowest-order behavior in a nice way.
% %
% We get something unpleasant:
% %
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.5\linewidth]{Figures/thrust_qcd.pdf}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}

% The full polynomial is:
% %
% \begin{align}
% p_{mn}(t) &= \begin{pmatrix}
% 0.00e+00 & -0.00e+00 & -0.00e+00 & -0.00e+00 & -0.00e+00 \\ 
% -6.37e-01 & 8.49e-01 & 0.00e+00 & 0.00e+00 & 6.32e-09 \\ 
% -8.62e-01 & 1.27e+00 & 1.59e+00 & -3.60e-01 & 0.00e+00 \\ 
% 0.00e+00 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 0.00e+00 \\ 
% 0.00e+00 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 0.00e+00 \end{pmatrix} \\
% &\downarrow \text{Shift} \nonumber \\
%    p_{mn}(t')  &= \begin{pmatrix}
% \tikzmark{left}{0.00e+00} & 0.00e+00 & -0.00e+00 & -0.00e+00 & -0.00e+00 \\ 
% 7.74e-06 & 8.49e-01 & -7.59e-08 & -2.53e-08 & 1.26e-08 \\ 
% 8.32e-01 & \tikzmark{right}{3.04e+00} & 7.77e-01 & -3.60e-01 & 1.29e-07 \\ 
% 0.00e+00 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 0.00e+00 \\ 
% 0.00e+00 & 0.00e+00 & 0.00e+00 & 0.00e+00 & 0.00e+00 \end{pmatrix}\Highlight[first]
% \end{align}


% I propose the following:
% %
% Originally, we chose $g^*$ to be just the lowest order term, and we divided it out so that the polynomial starts with 1.
% %
% Instead, we should divide out the lowest \emph{positive sub-block polynomial} (highlighted in red), and the entire thing can be $g^*$.
% %
% We have to do polynomial division to do this, but this can be done perturbatively.
% %
% This is a generalization of what we were already doing, where the sub-block is just a single term.
% %

% As an example, suppose we had:
% %
% \begin{align}
%     p = \alpha t + \alpha^2 (t + c),
% \end{align}
% %
% Which is a simplified version of the above case.
% %
% In matrix form,
% %
% \begin{align}
%     p = \begin{pmatrix}
% 0 & 0 & 0 \\ 
% 0 & 1 & 0 \\ 
% c & 1 & 0 \end{pmatrix}
% \end{align}
% %
% Naively, $g*$ can only be $\alpha$ here.
% %
% Running through our matching procedure above, we get:
% %
% \begin{align}
%     q = \alpha \exp{()}
% \end{align}




% %
% Naively, $g^*$ can only be $\alpha$ here.
% %
% However, if we choose $g^* = (\alpha + t)$, then the reduced polynomial is:
% %
% \begin{align}
%     p_{\rm reduced} &= 1 - \frac{\alpha^2 t^2}{\alpha + t} \nonumber \\
%     &\approx 1 - \alpha^2 t + \alpha^3
% \end{align}
% %
% so then, we have:
% %
% \begin{align}
%     q = (\alpha + t)\exp^{- \alpha^2 t + \text{stuff}}
% \end{align}




\section{Positive Polynomials}\label{app:polynomials}


Suppose we have a 2D polynomial:
%
\begin{align}
    f_c(t, \alpha) = \sum_{m,n} c_{mn} \alpha^m t^n. 
\end{align}
%
where $\alpha$ and $t$ are both positive, and $m, n \leq M, N$ is the degree of the polynomial. 
%
We also assume $\alpha$ is bounded above by $\alpha_{\max}$, which we may take to be infinite later.
%
Suppose also that some, but not all, of the $c_{mn}$ are frozen to pre-set values.
%
We would like this polynomial to be monotonic in $t$, which places constraints on the remaining unfrozen coefficients $c_{mn}$.

This is equivalent to asking that its $t$-derivative $f'(t, \alpha)$ (another polynomial) is positive everywhere, where the derivative has coefficients:
%
\begin{align}
    c_{m,n}' = (n+1)c_{m,n+1}. 
\end{align}
%
It will be more convenient to work in this primed basis, since it is simpler to think about positivity rather than monotonicity.\\


\noindent \textbf{Fact 1}: The lowest order nonzero $c'_{mn}$ must be positive. 

In the limit where $t\to 0$, only the terms with the lowest order in $n$ matter. Likewise, in the limit where $\alpha\to 0$, only the lowest order in $m$ matter. \Rikab{But what does ``lowest order'' mean precisely in a 2D polynomial? Vibes wise I know what I mean but I can't put it into math words} \Radha{The way you've explained is consistent with saying $c_{1n} \geq 0$ and $c_{m1} \geq 0$}\\

\noindent \textbf{Fact 2}: The highest order $c'_{mn}$ must be positive, if $\alpha_{\max} \to \infty$.

This fact follows from Fact 1, with the replacement $t \to \frac{1}{t}$ and $\alpha \to \frac{1}{\alpha}$. Since both $t$ and $\alpha$ are always positive, the resulting expression should still be positive.\\

\noindent \textbf{Fact 3}: For $N \leq 4$ only: define, for simplicity, $c'_n = \sum_m c_{mn}' \alpha^m$, which is the coefficient of the $t^n$.
%
Then the quartic polynomial discriminant:
%
\begin{align}
    \Delta_{c'} &= 256\,{c'_4}^{3}\,{c'_0}^{3}
- 192\,{c'_4}^{2}\,c'_3\,c'_1\,{c'_0}^{2}
- 128\,{c'_4}^{2}\,{c'_2}^{2}\,{c'_0}^{2}
+ 144\,{c'_4}^{2}\,c'_2\,{c'_1}^{2}\,c'_0
- 27\,{c'_4}^{2}\,{c'_1}^{4}\nonumber \\
\quad
&+ 144\,c'_4\,{c'_3}^{2}\,c'_2\,{c'_0}^{2}
- 6\,c'_4\,{c'_3}^{2}\,{c'_1}^{2}\,c'_0
- 80\,c'_4\,c'_3\,{c'_2}^{2}\,c'_1\,c'_0
+ 18\,c'_4\,c'_3\,c'_2\,{c'_1}^{3}
+ 16\,c'_4\,{c'_2}^{4}\,c'_0 \nonumber\\
&\quad - 4\,c'_4\,{c'_2}^{3}\,{c'_1}^{2}
- 27\,{c'_3}^{4}\,{c'_0}^{2}
+ 18\,{c'_3}^{3}\,c'_2\,c'_1\,c'_0
- 4\,{c'_3}^{3}\,{c'_1}^{3}
- 4\,{c'_3}^{2}\,{c'_2}^{3}\,c'_0
+ {c'_3}^{2}\,{c'_2}^{2}\,{c'_1}^{2}. 
\end{align}
%
cannot be negative, though this is not a sufficient condition.\Radha{Is this just copied from the Mathematica code? Or did you derive it another way?}
%
Further define:
%
\begin{align}
    \zeta_{c'} = 8 c'_4c_2' - 3{c'}_3^{2} 
\end{align}
%
A sufficient condition is $\Delta > 0$ and $\zeta > 0$ (strict inequalities). \\


\subsection{An attempt to derive positivity}

We have a function $f(\alpha, t) = \sum_{m=0}^M\sum_{n=0}^Nc_{mn}\alpha^m t^n$ that must be monotonic increasing, or $\sum_{mn}c_{mn}\alpha^m n t^{n-1} > 0$. Defining $R_n = \sum_m c_{mn}\alpha^m$, this condition becomes $\sum_n R_n n t^{n-1} > 0$. This must hold for any positive $t$, which means the equation must hold independently for all orders of $t$. So we have $N$ equations $\sum_m c_{mn}\alpha^m > 0$ for $n = 1$ to $N$ (note that all $n$ are positive, so they can be factored out).\\

\noindent Why must this hold independently for all $t$? Let's say we had $N = 3$, so we needed to solve $R_1 + 2R_2 t + 3R_3 t^2 > 0$. Let's say that we knew $R_1$ and $R_2$. So we would need to solve $R_3 = -\frac{R_1}{t^2}- 2\frac{R_2}{t}$. But this implies that $R_3$ is a function of $t$, which we don't want. \Rikab{I think this is false. We do not need to solve $R_3 = $ stuff. We would need to solve $R_3 \geq \max_t[-R_1/t^2 - R_2/t]$. This expression does not depend on $t$, since its maxed over. So since $R_3$ doesn't actually have to depend on t, the implication that the above stuff must be true independently for all $t$ does not follow.}\\

\noindent Example: say we know $c_{10}$, $c_{11}$, and $c_{20}$. i.e. we are given $f(\alpha, t)= c_{10}\alpha + c_{11}\alpha t +  c_{20} \alpha^2 $. Let's say we want to learn coefficients up to $M=4$, $N=4$.

\begin{itemize}
    \item For $n=0$, we have no equation. The constraints $c_{m0}$ are unconstrained by monotonicity and can only be determined through matching to data.
    \item For $n=1$, we have $c_{21}\alpha + c_{31}\alpha^2 + c_{41}\alpha^3 > c_{11} $ (we have divided out a common factor of $\alpha^1$)
    \item For $n=2$, we have $c_{12} + c_{22}\alpha + c_{32}\alpha^2 +c_{42}\alpha^3 > 0$
   \item For $n=3$, we have $c_{13} + c_{23}\alpha + c_{33}\alpha^2 +c_{43}\alpha^3 > 0$
    \item For $n=4$, we have $c_{14} + c_{24}\alpha + c_{34}\alpha^2 +c_{44}\alpha^3 > 0$
\end{itemize}

\noindent Now things get tricky -- the coefficients can't depend on $\alpha$ either, so we're left with nasty expressions for them...also, instead of having 1 overall positivity constraint, we now have $N$. 

\noindent \Radha{Really stupid idea: Let's say we carry out matching, then have a network learn the coefficients with the MSE loss. If we learn coefficients up to order $M$ in $\alpha$, can we simply add coefficients $c_{M+1, n}$ for each $n$ to satisfy positivity? So these coefficients would not be learned, but would be calculated after all network training. Since $\alpha$ is small, these coefficients should not affect the learned pdf too much...des  }



% \subsection{A completely general over-parameterization}

% \Rikab{@Radha, this is something I just kind of made up. Please let me know what you think?}

% I claim that the following is a parameterization of all $1D$ degree-$N$ polynomials $f'(t)$ that are positive for $t > 0$:
% %
% \begin{align}
%     f'(t) = \lambda \sum_{K = 0}^{\rm Floor(N/2)} \left(\prod_{i = 1}^K\left[(t - z_i^{(K)})(t - \bar{z}_i^{(K)})\right] \times \prod_{j = 0}^{N - 2K}\left[(t + a_j^{(K)})\right]  \right).
% \end{align}
% %
% where $z_i^{(K)}$ is a list of \emph{non-real} complex numbers, and $a_j^{(K)}$ is a list of $\emph{non-negative}$ real numbers, and $\lambda$ is a positive real number.
% %
% For any choice of these parameters, $f(t)$ will be positive for $t > 0$. 
% %
% However, note that there are more parameters than is typically expected in a 1D polynomial: a degree $N$ parameter has $N+1$ parameters, but my parameterization here has Floor($\frac{1}{2}N^2 + 1$) parameters. There is almost certainly some double counting. Maybe thats ok.\\

% \noindent \textbf{Sketch of proof}: By the Fundamental Theorem of Algebra, every polynomial can be written as a product of terms $(t-z_i)$ for complex $z$. 
% %
% The $z_i$ can be complex or real, even if the coefficients of the polynomial are solely real. 
% %
% However, for a real polynomial, if a root $z_i$ is complex, then its complex conjugate $\bar{z_i}$ must also be a root. 
% %
% Therefore, all polynomials can be written as:
% %
% \begin{align}
%     f'(t) = \lambda \prod_{i = 1}^K\left[(t - z_i)(t - \bar{z}_i)\right] \times \prod_{j = 0}^{N - 2K}\left[(t - a_j)\right],
% \end{align}
% %
% where $K$ is the number of complex-conjugate pairs, and $N-2K$ is the number of real roots. 
% %

% In this representation, it is easy to make sure the polynomial is positive for $t > 0$.
% %
% Step 1 is to make sure that the polynomial is positive \emph{somewhere} for $t > 0$. This is easy, just make $\lambda > 0$, so that $f'(\infty) = \infty$.
% %
% Step 2 is to make sure the polynomial never crosses zero, meaning it has no real roots for $t > 0$. This is easy: just don't let $a_j$ be positive and and sure $z_i$ are never strictly real.
% %
% Now $f'(t)$ is always positive. 
% %
% If we wanted $f'(t)$ to be positive everywhere instead of $t > 0$, it is even easier: we can forget about the $a$'s, and just have purely complex roots.

% But, a complication, which is that the number of real roots is a discrete object that we don't know ahead of time. 
% %
% That is, $(x-i)(x+i)(x+2)(x+3)$ cannot be reached by choosing $K = 2$ above. 
% %
% So, we simply sum over all possible choices of $K$. This is perfectly fine, since the sum of two polynomials that are positive over $t > 0$ is still positive. 


% There is a downside to this parameterization. Positivity is easy, but initialization is hard / inexact. It's not clear to me how to choose the $z_i$.
% %
% The $z_i$ have to be related somehow to $\sum c'_{mn} \alpha^m$ in a way that is extremeley non-obvious

% \subsection{Roots and $z$'s}


% Let's define the coefficient $c_n(\alpha) = \sum_{mn} c_{mn} \alpha^m$.
% %
% Then, $f(t, \alpha) = \sum_{n} c_n(\alpha) t^n$ is a 1D polynomial, and it has $N$ roots $z_n(\alpha)$.
% %
% As an example, if $f(t, \alpha) = 1 + 2\alpha t + t^2$, then $c_0 = 1, c_1 = 2\alpha$, and $c_2 = 1$, then the roots are:
% %
% \begin{align}
%     z_1(\alpha) &= -\alpha + \sqrt{\alpha^2 - 1}  \approx i - \alpha - \frac{i}{2}\alpha^2  \\
%     z_2(\alpha) &= -\alpha - \sqrt{\alpha^2 - 1} - \approx i - \alpha -+\frac{i}{2}\alpha^2
% \end{align}
% %
% The lesson is that even though the roots $z_n(\alpha)$ are not polynomials in $\alpha$, they \emph{approximately} are. So we can write $z_n(\alpha) = \sum A_{mn} \alpha^m$!

% Given a root $z_n(\alpha)$, is it easy to extract the coefficients $A_{mn}$?
% %
% To do this, we need the Taylor expansion, so we need to know $\frac{\partial^n z(\alpha)}{\partial\alpha^n}$.
% %
% I propose the following trick to automatically differentiate, without having to rely on numerical methods:
% %
% First, by definition of a root, we have:
% %
% \begin{align}
%     f(z(\alpha), \alpha) = 0
% \end{align}
% %
% Take the (full, not partial) derivative of both sides:
% %
% \begin{align}
%     0 &= \frac{d}{d\alpha} f(z(\alpha), \alpha) \\
%     &= \frac{d}{\partial\alpha} \sum_n c_n(\alpha) z^n(\alpha) \\
%     &= \sum_n \left[nc_n z^{n-1}(\alpha)\frac{d z(\alpha)}{d\alpha} + \frac{d c_n(\alpha)}{d\alpha}z^n \right] \\
%     &\downarrow\nonumber\\
%     \frac{d z(\alpha)}{d\alpha} &= - \frac{\sum_n \frac{d c_n(\alpha)}{d\alpha}z^n}{\sum_n nc_n z^{n-1}(\alpha)}
% \end{align}
% %
% We can write the RHS in terms of partial derivatives of $f(z, \alpha)$, where the $\alpha$-dependence of $z$ is ignored.
% %
% \begin{align}
%     \frac{d z(\alpha)}{d\alpha} = - \frac{ \frac{\partial}{\partial\alpha} f(t,\alpha)\eval_{t = z_\alpha} }{\frac{\partial}{\partial t} f(t,\alpha)\eval_{t = z_\alpha} }
% \end{align}
% %
% From here, its trivial to use autodiff to get higher derivatives. 
% %
% Then, to get the Taylor expansion (the $A_{mn}$ coeffs), we \emph{only} need to know $z(\alpha = 0)$, not all $\alpha$! 
% %
% Then, $z(\alpha)$ can be expressed as a polynomial in $\alpha$ using these derivatives, which depends only on the polynomial directly and not root solving.


\section{Useful Trick}

From 2104.06920, eq 4.8:

\begin{align}
    t(L) &\equiv \int_{\mu e^{-L}}^\mu \frac{d k_t}{k_t}\frac{\alpha_s(k_t)}{\pi} \\
    &= \frac{\log(1 - 2\alpha_s(\mu)\beta_0 L)}{2\pi \beta_0}
\end{align}
%
where $\beta_0 = \frac{11 C_A - 2n_f}{12\pi}$


